Adversarial Embedding: A robust and elusive Steganography and Watermarking technique

We propose adversarial embedding, a new steganography and watermarking technique that embeds secret information within images. The key idea of our method is to use deep neural networks for image classification and adversarial attacks to embed secret information within images. Thus, we use the attacks to embed an encoding of the message within images and the related deep neural network outputs to extract it. The key properties of adversarial attacks (invisible perturbations, nontransferability, resilience to tampering) offer guarantees regarding the confidentiality and the integrity of the hidden messages. We empirically evaluate adversarial embedding using more than 100 models and 1,000 messages. Our results confirm that our embedding passes unnoticed by both humans and steganalysis methods, while at the same time impedes illicit retrieval of the message (less than 13% recovery rate when the interceptor has some knowledge about our model), and is resilient to soft and (to some extent) aggressive image tampering (up to 100% recovery rate under jpeg compression). We further develop our method by proposing a new type of adversarial attack which improves the embedding density (amount of hidden information) of our method to up to 10 bits per pixel.

==> related_work.tex <==
\section{Related Work}
\label{sec:related}

%%% The content of this section should move elsewhere (in Sections 1-3)

Why we use adversarial attacks instead of direct models to embed data: \\
-Attacks allow to embed any message in any pictures, without needing to train a specific model for a specific message.
-Control the resilience of images to tampering is the attack process instead of the heavy model training process
-ensure that the classification is not transferable [targeted attacks have been demonstrated to be not transferable from custom model to another model]


How about using adversarial detectors to detect our watermarking?

Carlini and Wagner summarized most of these adversarial detecting methods ( [J. H. Metzen, T. Genewein, V. Fischer, and B. Bischoff, “On detecting adversarial perturbations,” Proceedings of5th International Conference on Learning Representations (ICLR), 2017.], [D. Hendrycks and K. Gimpel, “Early methods for detecting adversarial images,” ICLR Workshop, 2017.]) and showed that these methods could not defend against their previous attack C\&W’s Attack with slight changes of loss function [N. Carlini and D. Wagner, “Adversarial examples are not easily detected: Bypassing ten detection methods,” AISEC, 2017.]

